Same Question, Different Words: A Latent Adversarial Framework for Prompt Robustness

Insensitivity to semantically-preserving variations of prompts (paraphrases) is crucial for reliable behavior and real-world deployment of large language models. However, language models exhibit significant performance degradation when faced with semantically equivalent but differently phrased prompts, and existing solutions either depend on trial-and-error prompt engineering or require computationally expensive inference-time algorithms. In this study, built on the key insight that worst-case prompts exhibit a drift in embedding space, we present Latent Adversarial Paraphrasing (LAP), a dual-loop adversarial framework: the inner loop trains a learnable perturbation to serve as a "latent continuous paraphrase" while preserving semantics through Lagrangian regulation, and the outer loop optimizes the language model parameters on these perturbations. We conduct extensive experiments to demonstrate the effectiveness of LAP across multiple LLM architectures on the RobustAlpaca benchmark with a 0.5%-4% absolution improvement on worst-case win-rate compared with vanilla supervised fine-tuning.

==> feedback.tex <==
feedback from ryko
Hi Fazl,
Thank you for the opportunity of our great chat last week.
Here is my feedback/review of the shared paper. (Sorry for that this might include my misunderstanding, in advance)
Strengths:
The paper is very well written and easy to follow.
The motivation of their work is clear: To adopt Latent Adversarial Training (LAT) to improve the prompt robustness of LLMs, they add the constraint on the semantic distance (language modeling loss) to LAT and apply the Lagrange multiplier to optimize the perturbation under the constraint.
The main results show the superior performance of LAP than baseline algorithms on the multiple paraphrased prompts using the RobustAlpaca benchmark. Besides, they offer a thorough analysis of various aspects of their proposed method.
Weaknesses:
I have a concern about the main results.
While the average and best winrates have increased, the worst winrate—which is likely the most important to improve—has not much compared to prior methods. Thus, in addition to the results of best, worst, and average, it would be useful to examine whether the performance has improved overall for samples with large L2 distances, as shown in Figure 3.
Currently, the improvement in average performance might be due to improvements in samples with small L2 distances or original samples, raising a concern that the improvement for samples with large L2 distances may not have been achieved.
Comments and Questions:
Adding some information on datasets used for experiments would help readers’ understanding:
The information (e.g., the number of training samples and train/valid/test split) about the dataset used for training base models are missing
In the description of the tasks in RobustAlpaca (based on TinyAlpaca), it is unclear which tasks LAP improved performance on
How is the threshold ε determined? Is it when performance on the dev set is maximized?
According to Table 5, the phenomenon where the worst win rate is slower to improve compared to the best win rate or average rate is reversed in larger models like the 13B model. Is this because the model size has increased, or is it simply due to differences between the models, similar to how the original win rate of SFT varies significantly between Llama and Mistral in Table 1?
Typos:
In Table 1, the second-best model in the worst winrate of Llama-3-8b seems to be wrong; not LAP (1.99) but LAT (2.04)
In section 3.1., “with the inserted perturbation after layer i → layer l,”
In the section of ‘Experimental results’, “a large margin between the best win-rate and the worst win-ratel → win-rate”
Best,
Ryuto
